Intrinsically-Typed Mechanized Semantics for Session Types

Session types have emerged as a powerful paradigm for structuring communication-based programs. They guarantee type soundness and session fidelity for concurrent programs with sophisticated communication protocols. As type soundness proofs for languages with session types are tedious and technically involved, it is rare to see mechanized soundness proofs for these systems. We present an executable intrinsically typed small-step semantics for a realistic functional session type calculus. The calculus includes linearity, recursion, and recursive sessions with subtyping. Asynchronous communication is modeled with an encoding. The semantics is implemented in Agda as an intrinsically typed, interruptible CEK machine. This implementation proves type preservation and a particular notion of progress by construction.

==> AlternativeMatch3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{AlternativeMatch3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{-- open import Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Channel3}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Session3}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{TypeReduction3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G₁′}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{R₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{R₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{RedEnd}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedEnd}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{R₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{R₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{R₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- find matching wait instruction in thread pool}\<%
\end{code}
%<*vcr-match>
\begin{code}%
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\end{code}
%</vcr-match>
%<*vcr-match-body>
\begin{code}%
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr2}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{map}%
\>[287I]\AgdaSymbol{(λ\{}%
\>[288I]\AgdaSymbol{(}\AgdaBound{b≡}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
\>[.][@{}l@{}]\<[288I]%
\>[10]\AgdaSymbol{(}\AgdaBound{b≡}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{\})}\<%
\\
\>[.][@{}l@{}]\<[287I]%
\>[6]\AgdaSymbol{(}\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedEnd}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedEnd}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{))}\<%
\end{code}
%</vcr-match-body>
%<*matchWaitAndGo>
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- close command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\end{code}
%</matchWaitAndGo>
--   → Maybe (Σ SCtx λ G′ → G ⇒′ G′ × ThreadPool G′)
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\end{code}
%<*matchWaitAndGo-new>
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\<%
\\
%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\end{code}
%</matchWaitAndGo-new>
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaBound{ss-g3gi′}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaBound{w-vcr}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}\{}\AgdaArgument{Gc₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b≡}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gchannel′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gc}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{Gc₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{extract-inactive-from-cont}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped′}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-int}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaBound{ss-int}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{lift-reduce}\AgdaSpace{}%
\AgdaBound{ss-top′}\AgdaSpace{}%
\AgdaBound{R}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gout}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-out}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Rout}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss-out}\AgdaSpace{}%
\AgdaBound{ina-Gc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Rout}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)))))}\<%
\end{code}
%<*vcr-match-2-sr>
\begin{code}%
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}%
\>[996I]\AgdaSymbol{(}\AgdaBound{b₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
\>[.][@{}l@{}]\<[996I]%
\>[10]\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[10]\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\end{code}
%</vcr-match-2-sr>
\begin{code}%
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[208]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SRecv}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SSend}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedTransmit}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}%
\>[97]\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- read command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-arg}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}%
\>[86]\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}%
\>[75]\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSymbol{@(}\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi′gig2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi′′gi′gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi′′}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gg1′g2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1′gc1g11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2′gc2gi′′}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-gg1′g2′}\AgdaSpace{}%
\AgdaBound{ss-g1′gc1g11}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaBound{vcr}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaComment{\{-t1≡t-\}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1≡s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-out1}\AgdaSpace{}%
\AgdaBound{ss-out2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′GG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gi′′gi′gtpacc}\AgdaSpace{}%
\AgdaBound{ss-gi′gig2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GSi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi′′GiGi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi1G2Gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-out1}\AgdaSpace{}%
\AgdaBound{ss-out2}\AgdaSpace{}%
\AgdaBound{ss-g2′gc2gi′′}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GG1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1′-GG2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG1′-GG11-Gc2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2′-G12-Gi′′}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-rotate}\AgdaSpace{}%
\AgdaBound{ss-GG2′-G12-Gi′′}\AgdaSpace{}%
\AgdaBound{ss-Gi′′GiGi1}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′′+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2-G12-Gi′′+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi′′+Gi+Gsi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi+-G12-G4}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1′-GG2′}\AgdaSpace{}%
\AgdaBound{ss-GG1′-GG11-Gc2}\AgdaSpace{}%
\AgdaBound{ss-GG2-G12-Gi′′+}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GG1′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG2′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1′′-GG2′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG1′′-GG11-G12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2′′-Gc2-Gi′′+}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1′′-GG2′′}\AgdaSpace{}%
\AgdaBound{ss-GG2′′-Gc2-Gi′′+}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-Gii-Gi′′+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gii-GG1′′-Gc2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-GG-Gii-Gi′′+}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-Gii-GG1′′-Gc2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-GG1′′-GG11-G12}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-Gi′′+Gi+Gsi}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-Gi+-G12-G4}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-Gi1G2Gtpacc}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSymbol{@(}\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi′gig2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi′′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi′′gi′gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gg1′g2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1′gc1g11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2′gc2gi′′}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\end{code}

\begin{code}%
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}%
\>[2531I]\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
\>[.][@{}l@{}]\<[2531I]%
\>[10]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[10]\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSpace{}%
\AgdaBound{ss2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-int′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-ext′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SIntern}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SExtern}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[193]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[194]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChLeft}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedChRight}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₁′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₂′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSpace{}%
\AgdaBound{ss2′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-int′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-ext′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaBound{R}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- select command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc′-gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc′-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp′-gc2-gi1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-g-gc′-gtp′}\AgdaSpace{}%
\AgdaBound{ss-gc′-gc1-g1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSymbol{@(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc′-gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc′-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp′-gc2-gi1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gix}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp′}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss′}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc′-gtp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc′-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp′-gc2-gi1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds3=s1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds4=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSpace{}%
\AgdaBound{ss2′}%
\>[332]\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-sel}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-bra}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{R₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′GG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-g3-gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi2-g2-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss1′}\AgdaSpace{}%
\AgdaBound{ss2′}\AgdaSpace{}%
\AgdaBound{ss-gtp′-gc2-gi1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GGG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GGG2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-ggg1-ggg2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg1-gc1-gc2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-g1-gi1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-g1-gi1}\AgdaSpace{}%
\AgdaBound{ss-gi1-g3-gi2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-gi3-gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi3-gg12-g2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-GG-ggg1-ggg2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-ggg1-gc1-gc2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr-sel}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-ggg2-gi3-gi2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-gi3-gg12-g2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr-bra}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{dcont}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-gi2-g2-gtpacc}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- -\}}\<%
\\
\>[0]\AgdaComment{-- -\}}\<%
\\
\>[0]\AgdaComment{-- -\}}\<%
\\
\>[0]\AgdaComment{-- -\}}\<%
\\
\>[0]\AgdaComment{-- -\}}\<%
\end{code}


==> Async3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Async3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{drop}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
\>[0]\AgdaComment{-- open import Values3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaBound{φ}\<%
\\
\>[0]\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{φ}\AgdaSpace{}%
\AgdaBound{φ}\<%
\\
\>[0]\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{px}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{un-φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{px}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{un-φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-
-- an asynchronous channel is a promise for a channel
AChan : STy → Ty
AChan s = TChan (SRecv (TChan s) SEnd!)
-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- create an async channel}\<%
\end{code}
%<*async-anew>
\begin{code}%
\>[0]\AgdaFunction{anew}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)))}\<%
\end{code}
%</async-anew>
\begin{code}%
\>[0]\AgdaFunction{anew}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[148I]\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))))))}\<%
\\
\>[.][@{}l@{}]\<[148I]%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{fork}%
\>[156I]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[156I]%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[172I]\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))))))}\<%
\\
\>[.][@{}l@{}]\<[172I]%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{fork}%
\>[179I]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[179I]%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{))))}\<%
\\
%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-unr}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)))))))))}\<%
\end{code}
%<*async-asend>
\begin{code}%
\>[0]\AgdaFunction{asend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vt}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\end{code}
%</async-asend>
\begin{code}%
\>[0]\AgdaFunction{asend}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{vt}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[261I]\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)))}\<%
\\
\>[.][@{}l@{}]\<[261I]%
\>[11]\AgdaComment{-- read actual channel \& actual send \& send depleted channel \& close}\<%
\\
%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{fork}%
\>[265I]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[265I]%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vt}\AgdaSymbol{)}\<%
\\
%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[293I]\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))}\<%
\\
\>[.][@{}l@{}]\<[293I]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))}\<%
\\
%
\>[17]\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))))))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- receive is a blocking operation!}\<%
\end{code}
%<*async-arecv>
\begin{code}%
\>[0]\AgdaFunction{arecv}%
\>[313I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[.][@{}l@{}]\<[313I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\end{code}
%</async-arecv>
\begin{code}%
\>[0]\AgdaFunction{arecv}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-right}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[388I]\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))}\<%
\\
\>[.][@{}l@{}]\<[388I]%
\>[11]\AgdaSymbol{(}\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}%
\>[394I]\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[394I]%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[26]\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)))))))))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{aclose}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
\>[0]\AgdaFunction{aclose}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{fork}%
\>[430I]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[430I]%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{await}%
\>[449I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[.][@{}l@{}]\<[449I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
\>[0]\AgdaFunction{await}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{fork}%
\>[463I]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{split-all-left}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[463I]%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{)}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))}\<%
\\
%
\>[7]\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSymbol{))))))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{\{-
anselect : ∀ \{Φ m alt\}
      → (lab : Fin m)
      → (ch : AChan (sintN m alt) ∈ Φ)
      → Expr Φ (AChan (alt lab))
anselect \{alt = alt\} lab ch =
  letbind (split-all-right \AgdaUnderscore{})
          (new [] (SRecv (TChan (alt lab)) SEnd!))
  (letpair (left (split-all-right \AgdaUnderscore{})) (here [])
  (letbind (rght (left (split-all-left \AgdaUnderscore{})))
           (fork (letbind (rght (split-all-left \AgdaUnderscore{})) (recv ch)
                 (letpair (left (rght [])) (here [])
                 (letbind (left (rght (rght []))) (close (here []))
                 (letbind (drop UUnit (left (rght []))) (nselect lab (here []))
                 (letbind (left (left [])) (send (rght (left [])) (here []) (here []))
                 (wait (here []))))))))
  (var (there UUnit (here [])))))

-- branching is a blocking operation!
anbranch : ∀ \{Φ m alt Φ₁ Φ₂ t\}
      → (sp : Split Φ Φ₁ Φ₂)
      → (ch : AChan (sextN m alt) ∈ Φ₁)
      → (ealts : (i : Fin m) → Expr (AChan (alt i) ∷ Φ₂) t)
      → Expr Φ t
anbranch\{alt = alt\} sp ch ealts =
  letbind sp (recv ch)
  (letpair (left (split-all-right \AgdaUnderscore{})) (here [])
  (letbind (left (split-all-right \AgdaUnderscore{})) (close (here []))
  (nbranch (drop UUnit (left (split-all-right \AgdaUnderscore{}))) (here [])
  (λ i → letbind (split-all-right \AgdaUnderscore{}) (new [] (SRecv (TChan (alt i)) SEnd!))
         (letpair (left (split-all-right \AgdaUnderscore{})) (here [])
         (letbind (rght (left (left (split-all-right \AgdaUnderscore{})))) 
                  (fork (letbind (left (left [])) (send (left (rght [])) (here []) (here []))
                        (wait (here [])))) 
         (letbind (drop UUnit (left (split-all-right \AgdaUnderscore{}))) (var (here []))
                  (ealts i))))))))
-\}}\<%
\end{code}


==> Channel3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Channel3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaComment{-- open import Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- the main part of a channel endpoint value is a valid channel reference}\<%
\\
\>[0]\AgdaComment{-- the boolean determines whether it's the front end or the back end of the channel}\<%
\\
\>[0]\AgdaComment{-- enforces that the session context has only one channel}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ce}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\>[2]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vcr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- find matching wait instruction in thread pool}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSpace{}%
\AgdaBound{vcr2}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{vcr-there}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
\>[0]\AgdaFunction{vcr-there}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- find matching send instruction in thread pool}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}%
\>[282I]\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
\>[.][@{}l@{}]\<[282I]%
\>[10]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[10]\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁≡t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{s₁≡ds₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁≡t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{s₁≡ds₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{vcr-there}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- ok. brute force for a fixed tree with three levels}\<%
\end{code}
%<*SSplit2>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaBound{ss1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\end{code}
%</SSplit2>
%<*vcr-match-2-sr>
\begin{code}%
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}%
\>[562I]\AgdaSymbol{(}\AgdaBound{b₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
\>[.][@{}l@{}]\<[562I]%
\>[10]\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[10]\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\end{code}
%</vcr-match-2-sr>
\begin{code}%
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[283]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SRecv}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SSend}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)))))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}%
\>[97]\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b1=nb2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{t1=t2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss3}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss4}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-send}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}%
\>[1501I]\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
\>[.][@{}l@{}]\<[1501I]%
\>[10]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaSymbol{→}\<%
\\
%
\>[10]\AgdaDatatype{Junction}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁₁}\AgdaSpace{}%
\AgdaBound{s₁₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\<%
\\
%
\>[10]\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₂₁}\AgdaSpace{}%
\AgdaBound{s₂₂}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSpace{}%
\AgdaBound{ss2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-int'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-ext'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SIntern}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{SExtern}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[193]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[194]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-inv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₁₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSpace{}%
\AgdaBound{ss2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-int'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-ext'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds11=s21}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds12=s22}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext'}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{vcr-ext}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr-int}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{lab}\<%
\end{code}


==> Extension3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Extension3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- open import Typing3 hiding (dual)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaInductiveConstructor{recv}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Session3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{LU}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{LL}\AgdaSpace{}%
\AgdaInductiveConstructor{UU}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{LU}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Act0}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[1][@{}l@{\AgdaIndent{0}}]%
\>[3]\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Act1}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
%
\>[1]\AgdaKeyword{postulate}\<%
\\
\>[1][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{SChoice}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cases}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\end{code}
%<*SChoice>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{SSelect}\AgdaSpace{}%
\AgdaInductiveConstructor{SBranch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cases}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\end{code}
%</SChoice>
\begin{code}%
%
\>[1]\AgdaKeyword{postulate}\<%
\end{code}
%<*Function>
\begin{code}%
\>[1][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{TFun}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{LU}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\end{code}
%</Function>
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Act2}\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
%
\>[1]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Act1}\<%
\\
%
\>[1]\AgdaKeyword{postulate}\<%
\end{code}
%<*SChoice-syntax>
\begin{code}%
\>[1][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{nselect}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSelect}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{nbranch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SBranch}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cases}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</SChoice-syntax>
%<*Function-syntax>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{llambda}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{body}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TFun}\AgdaSpace{}%
\AgdaInductiveConstructor{LL}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{rec}%
\>[174I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[.][@{}l@{}]\<[174I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}%
\>[183I]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{TFun}\AgdaSpace{}%
\AgdaInductiveConstructor{UU}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
\>[.][@{}l@{}]\<[183I]%
\>[8]\AgdaSymbol{(}\AgdaBound{body}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</Function-syntax>
%<*Function-syntax-app>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{app}%
\>[202I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{lu}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[202I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{fun}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TFun}\AgdaSpace{}%
\AgdaBound{lu}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{arg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\end{code}
%</Function-syntax-app>
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Act3}\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[1]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
%
\>[1]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Act1}\<%
\\
%
\>[1]\AgdaKeyword{postulate}\<%
\end{code}
%<*SChoice-commands>
\begin{code}%
\>[1][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{NSelect}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSelect}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaInductiveConstructor{NBranch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SBranch}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{dcont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</SChoice-commands>
\begin{code}%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaModule{Act0}\<%
\\
\>[0]\AgdaKeyword{mutual}\<%
\end{code}
%<*rectypes>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\\
%
\>[4]\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\\
%
\>[4]\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\\
%
\>[4]\AgdaInductiveConstructor{TFun}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{LU}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\<%
\\
\>[0]\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{S}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{stransmit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{S}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaBound{S}\<%
\\
%
\>[4]\AgdaInductiveConstructor{schoice}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ℕ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{S}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaBound{S}\<%
\\
%
\>[4]\AgdaInductiveConstructor{end}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaBound{S}\<%
\end{code}
%</rectypes>
%<*rectypes-1>
\begin{code}%
%
\>[2]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaKeyword{coinductive}\<%
\\
%
\>[4]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{force}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaRecord{SType}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{stransmit}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\>[2]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}%
\>[21]\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{stransmit}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\>[2]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{sint}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{schoice}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\<%
\\
%
\>[2]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{sext}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{schoice}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\<%
\end{code}
%</rectypes-1>
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Act4}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Expr'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\>[2]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{SType}\<%
\\
%
\>[2]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\>[2]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Inner}\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaKeyword{postulate}\<%
\end{code}
%<*rectypes-new>
\begin{code}%
\>[4][@{}l@{\AgdaIndent{1}}]%
\>[6]\AgdaInductiveConstructor{new}%
\>[446I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[446I]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr'}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}%
\>[459I]\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{SType.force}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[459I]%
\>[27]\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{SType.force}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))))}\<%
\end{code}
%</rectypes-new>
%<*rectypes-sub>
\begin{code}%
\>[0]\AgdaKeyword{mutual}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaComment{-- subtyping}\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Type}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{sub-unit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-pair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-fun}%
\>[13]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSpace{}%
\AgdaBound{lu}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TFun}\AgdaSpace{}%
\AgdaBound{lu}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TFun}\AgdaSpace{}%
\AgdaBound{lu}\AgdaSpace{}%
\AgdaBound{t₁′}\AgdaSpace{}%
\AgdaBound{t₂′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-chan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaRecord{Sub}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{s′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s′}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaComment{-- session type subtyping}\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STF}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{sub-send}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s1}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t′≤t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s1≤s1′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-recv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s1}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t≤t′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SubT}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s1≤s1′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSymbol{)}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{t′}\AgdaSpace{}%
\AgdaBound{s1′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-sint}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{alt′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m′≤m}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inject≤}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaBound{m′≤m}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt′}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{))}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{sint}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{sint}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSpace{}%
\AgdaBound{alt′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-sext}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{alt′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{m≤m′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≤}}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaBound{i}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Fin}\AgdaSpace{}%
\AgdaBound{m}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt}\AgdaSpace{}%
\AgdaBound{i}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{alt′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inject≤}\AgdaSpace{}%
\AgdaBound{i}\AgdaSpace{}%
\AgdaBound{m≤m′}\AgdaSymbol{)))}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{sext}\AgdaSpace{}%
\AgdaBound{m}\AgdaSpace{}%
\AgdaBound{alt}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{sext}\AgdaSpace{}%
\AgdaBound{m′}\AgdaSpace{}%
\AgdaBound{alt′}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{sub-end}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{d}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaBound{R}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{end}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{end}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaKeyword{record}\AgdaSpace{}%
\AgdaRecord{Sub}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s′}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaRecord{SType}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaKeyword{coinductive}\<%
\\
%
\>[4]\AgdaKeyword{field}\AgdaSpace{}%
\AgdaField{force}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SubF}\AgdaSpace{}%
\AgdaRecord{Sub}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{SType.force}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaField{SType.force}\AgdaSpace{}%
\AgdaBound{s′}\AgdaSymbol{)}\<%
\end{code}
%</rectypes-sub>


==> Global0.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Global0}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe.Relation.Unary.All}\AgdaSpace{}%
\AgdaKeyword{renaming}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{All}\AgdaSpace{}%
\AgdaSymbol{to}\AgdaSpace{}%
\AgdaDatatype{MAll}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing0}\<%
\end{code}
Global session context
%<*SCtx>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{PosNeg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{PosNeg}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{Session}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{PosNeg}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaFunction{Session}\<%
\end{code}
%</SCtx>
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{MySplitting}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}
%<*RSplit>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{Session}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Session}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Session}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{rs-both}%
\>[14]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[4]\AgdaInductiveConstructor{rs-left}%
\>[14]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
%
\>[4]\AgdaInductiveConstructor{rs-right}%
\>[14]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaInductiveConstructor{rs-posneg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{\}}%
\>[26]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}%
\>[78I]\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[78I]%
\>[35]\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{))}\<%
\\
%
\>[4]\AgdaInductiveConstructor{rs-negpos}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{\}}%
\>[26]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}%
\>[95I]\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[95I]%
\>[35]\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{))}\<%
\end{code}
%</RSplit>
%<*SSplit2>
\begin{code}%
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[4]\AgdaInductiveConstructor{ss-::}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\end{code}
%</SSplit2>
%<*ssplit-sym>
\begin{code}%
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{RSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-both}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-both}\<%
\\
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-right}\<%
\\
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-left}\<%
\\
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-posneg}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-negpos}\<%
\\
%
\>[2]\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-negpos}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{rs-posneg}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
%
\>[2]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
%
\>[2]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-::}\AgdaSpace{}%
\AgdaBound{rs}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{rsplit-sym}\AgdaSpace{}%
\AgdaBound{rs}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\end{code}
%</ssplit-sym>
-- SSplit G G₁ G₂
-- split G into G₁ and G₂
-- length and position preserving
%<*SSplit>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ss-[]}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ss-both}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}%
\>[18]\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[11]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ss-left}%
\>[11]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[11]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ss-right}%
\>[264I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[.][@{}l@{}]\<[264I]%
\>[11]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{spn}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}%
\>[19]\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}%
\>[19]\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[10]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\end{code}
%</SSplit>
\begin{code}%
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- tedious but easy to prove}\<%
\end{code}
%<*ssplit-compose>
\begin{code}%
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\end{code}
%</ssplit-compose>
\begin{code}%
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[30]\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[26]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\\
\>[0]\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₂₄}\<%
\end{code}
%<*ssplit-compose2>
\begin{code}%
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSymbol{)}\<%
\end{code}
%</ssplit-compose2>
\begin{code}%
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
\>[0]\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssy}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssy}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
\>[0]\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss234}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaBound{ss12}\AgdaSpace{}%
\AgdaBound{ss234}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssi13}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssi4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssi13}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-compose4}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{[]}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POSNEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{NEG}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{.(}}\AgdaDottedPattern{\AgdaInductiveConstructor{just}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{(\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaInductiveConstructor{POS}}\AgdaDottedPattern{\AgdaSymbol{)}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaOperator{\AgdaInductiveConstructor{∷}}}\AgdaSpace{}%
\AgdaDottedPattern{\AgdaSymbol{\AgdaUnderscore{})}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-21i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-122}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-compose5}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
\>[0]\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-112}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-112}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-compose6}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
\>[0]\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-g11i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-g122}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-join}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSymbol{\}}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaBound{G₂₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₂₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{G₂₂}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[94]\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[2937I]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[2937I][@{}l@{\AgdaIndent{0}}]%
\>[48]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
%
\>[48]\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[3054I]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[3054I][@{}l@{\AgdaIndent{0}}]%
\>[48]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[3092I]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[3092I][@{}l@{\AgdaIndent{0}}]%
\>[48]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
%
\>[48]\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[3328I]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[3328I][@{}l@{\AgdaIndent{0}}]%
\>[48]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
%
\>[48]\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
\>[0]\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-2122}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[3486I]\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[3486I][@{}l@{\AgdaIndent{0}}]%
\>[48]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
%
\>[48]\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-1121}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-2122}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- a session context is inactive if all its entries are void}\<%
\end{code}
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{MyInactive}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[4]\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\end{code}
%<*Inactive>
\begin{code}%
%
\>[2]\AgdaFunction{Inactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\<%
\\
%
\>[2]\AgdaFunction{Inactive}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaFunction{Is-nothing}\<%
\end{code}
%</Inactive>
\begin{code}%
%
\>[2]\AgdaFunction{ina-ina-equiv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaFunction{ina-ina-equiv}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\<%
\\
%
\>[2]\AgdaFunction{ina-ina-equiv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ina-ina-equiv}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaFunction{ina'-ina-equiv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive'}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaFunction{ina'-ina-equiv}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaFunction{ina'-ina-equiv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDottedPattern{\AgdaSymbol{.}}\AgdaDottedPattern{\AgdaInductiveConstructor{nothing}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina'G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Data.Maybe.Relation.Unary.All.All.nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaFunction{ina'-ina-equiv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{ina'G}\<%
\end{code}
%<*Inactive-orig>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\end{code}
%</Inactive-orig>
\begin{code}%
\>[0]\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina1}\AgdaSpace{}%
\AgdaBound{ina2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{ina2}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ina1}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\AgdaSpace{}%
\AgdaBound{ina2}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ina1}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-left}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\end{code}
%<*ssplit-refl-left-inactive>
\begin{code}%
\>[0]\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\<%
\end{code}
%</ssplit-refl-left-inactive>
\begin{code}%
\>[0]\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-GG'}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-GG'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\\
\>[0]\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp'}\<%
\end{code}
%<*inactive-left-ssplit>
\begin{code}%
\>[0]\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\end{code}
%</inactive-left-ssplit>
\begin{code}%
\>[0]\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{inG₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{inG₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{inG₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{inG₁}\AgdaSymbol{)}\<%
\end{code}
%<*inactive-right-ssplit>
\begin{code}%
\>[0]\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\end{code}
%</inactive-right-ssplit>
\begin{code}%
\>[0]\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{inactive-right-ssplit-sym}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-sym}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G'}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-G'G1G2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₁'}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function1}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1'G2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₂'}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-right}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{cong}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{}∷\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2'}\AgdaSymbol{)}\<%
\end{code}


==> ProcessSyntax3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{ProcessSyntax3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} processes}\<%
\end{code}
%<*proc-data>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{exp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{par}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{res}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{P}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{))}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Proc}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\end{code}
%</proc-data>


==> Schedule3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Schedule3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function}\AgdaSpace{}%
\AgdaKeyword{using}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}\$\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Channel3}\<%
\\
\>[0]\AgdaComment{-- open import Values}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Session3}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaDatatype{Outcome}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{start}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaSymbol{;}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{TypeReduction3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{AlternativeMatch3}\<%
\end{code}

-- Event: outcomes of step
-- Gas: stuff to run
-- Outcome: outcomes of scheduling
%<*scheduler-event>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Event}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaInductiveConstructor{Forked}\AgdaSpace{}%
\AgdaInductiveConstructor{Restarted}\AgdaSpace{}%
\AgdaInductiveConstructor{Halted}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Event}\<%
\\
%
\>[2]\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaInductiveConstructor{Closed}\AgdaSpace{}%
\AgdaInductiveConstructor{Received}\AgdaSpace{}%
\AgdaInductiveConstructor{Stuck}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Event}\<%
\end{code}
%</scheduler-event>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{Selected}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Event}\<%
\end{code}
%<*scheduler-nextpool>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{NextPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[\AgdaUnderscore{},\AgdaUnderscore{},\AgdaUnderscore{}]]}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Event}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G′}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{NextPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</scheduler-nextpool>
%<*scheduler-types>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\\
%
\>[2]\AgdaInductiveConstructor{More}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Outcome}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaInductiveConstructor{Stuck}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{\AgdaUnderscore{},\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Event}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
%
\>[2]\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\end{code}
%</scheduler-types>
%<*step>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{NextPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{@(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{@(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Stuck}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}%
\>[191I]\AgdaInductiveConstructor{Restarted}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[.][@{}l@{}]\<[191I]%
\>[5]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{inaG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{inaG}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Halted}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\end{code}
%</step>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaArgument{G₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G2unit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Forked}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[268I]\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSymbol{)}\<%
\\
\>[268I][@{}l@{\AgdaIndent{0}}]%
\>[27]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\end{code}
%<*step-new>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}%
\>[307I]\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedNew}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\<%
\\
\>[.][@{}l@{}]\<[307I]%
\>[5]\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{((}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\\
\>[5][@{}l@{\AgdaIndent{0}}]%
\>[9]\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}%
\>[316I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\AgdaSymbol{)}\<%
\\
\>[316I][@{}l@{\AgdaIndent{0}}]%
\>[18]\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}%
\>[318I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[318I]%
\>[25]\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\<%
\\
%
\>[25]\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{)))}\<%
\\
%
\>[18]\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{))}\<%
\\
%
\>[9]\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)))}\<%
\\
%
\>[9]\AgdaSymbol{(}\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\end{code}
%</step-new>
%<*step-close>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{Gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG′}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}%
\>[359I]\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG′}\<%
\\
\>[.][@{}l@{}]\<[359I]%
\>[22]\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tpnext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Closed}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedInternal}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tpnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\end{code}
%</step-close>
%<*step-wait>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\end{code}
%</step-wait>
%<*step-send>
\begin{code}%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{Gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG′}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Received}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedInternal}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{Gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG′}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG′}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaInductiveConstructor{Selected}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{RedInternal}\AgdaSpace{}%
\AgdaBound{G⇒′Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1′}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2′}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-top1}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-top2}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\end{code}
%<*single-step>
\begin{code}%
\>[0]\AgdaFunction{single-step}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Event}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{single-step}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG′}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{step}\AgdaSpace{}%
\AgdaBound{ss-GG′}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G′}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{[[}}\AgdaSpace{}%
\AgdaBound{ev}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{red}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp′}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{]]}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ev}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp′}\<%
\end{code}
%</single-step>
-- thread scheduling
%<*schedule>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaBound{tp}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{gas}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{single-step}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Terminated}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{Stuck}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp′}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Stuck}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaSymbol{...}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaSymbol{|}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{ev}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaSymbol{\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaOperator{\AgdaInductiveConstructor{,}}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{tp′}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ev}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{gas}\AgdaSpace{}%
\AgdaBound{tp′}\<%
\end{code}
%</schedule>
\begin{code}%
\>[0]\AgdaComment{-- start main thread}\<%
\end{code}
%<*start>
\begin{code}%
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaKeyword{let}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{decompose}%
\>[741I]\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[741I]%
\>[18]\AgdaSymbol{(}\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{))}\<%
\\
%
\>[2]\AgdaKeyword{in}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{))}\<%
\end{code}
%</start>


==> Session0.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Session0}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{reverse}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaDeadcode{\AgdaKeyword{open}}\AgdaSpace{}%
\AgdaDeadcode{\AgdaKeyword{import}}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing0}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax0}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global0}\<%
\\
\>[0]\<%
\end{code}
-- the main part of a channel endpoint value is a valid channel reference
-- the boolean determines whether it's the front end or the back end of the channel
-- enforces that the session context has only one channel
%<*ChannelRef>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{po}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\>[2]\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{s}\<%
\end{code}
%</ChannelRef>
-- a value indexed by a *relevant* session context, which is "used up" by the value
%<*Val>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{po}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{po}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\end{code}
%</Val>
\begin{code}%
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[16]\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{unrt₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt₁}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- type environment-indexed value environment}\<%
\\
\>[0]\AgdaComment{-- session context G describes the entire environment, it splits over all (channel) values}\<%
\end{code}
%<*VEnv>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\end{code}
%</VEnv>
\begin{code}%
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{px}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{px}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- access a value in an indexed environment}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{allUnr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[40]\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{allUnr}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{inaG₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{inaG₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ssp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ssp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- split environment according to type context split}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSymbol{\{}\AgdaArgument{G}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[34]\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi-1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GGiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[2]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{p₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[17]\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p₂}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSymbol{\{}\AgdaArgument{G}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1'Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1'Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\\
%
\>[2]\AgdaInductiveConstructor{More}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\end{code}
%<*Cont>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}%
\>[32]\AgdaComment{-- all resources used up}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{un-t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}%
\>[32]\AgdaComment{-- return value is unrestricted}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ts}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}%
\>[32]\AgdaComment{-- split variables}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}%
\>[32]\AgdaComment{-- split ressources}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}%
\>[32]\AgdaComment{-- abstract from argument t}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</Cont>
%<*Command>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\end{code}
%</Command>
%<*Command-Halt>
\begin{code}%
\>[0][@{}l@{\AgdaIndent{1}}]%
\>[2]\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Halt>
%<*Command-Ready>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}%
\>[32]\AgdaComment{-- split resources}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}%
\>[32]\AgdaComment{-- intention: invoke (κ v)}\<%
\end{code}
%</Command-Ready>
%<*Command-Fork>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Fork>
%<*Command-New>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))))}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-New>
%<*Command-Close>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Close>
%<*Command-Wait>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{Wait}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Wait>
\begin{code}%
\>[0]\AgdaFunction{rewrite-helper}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaBound{Φ'}\<%
\\
\>[0]\AgdaFunction{rewrite-helper}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GGG''}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ina-G2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{sym}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp-GGG''}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{decompose-one}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{tin}\AgdaSpace{}%
\AgdaBound{tout}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{tin}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{tout}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tsp-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{tin}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{tout}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%<*decompose-one>
\begin{code}%
\>[0]\AgdaFunction{decompose-one}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tsp-Φ}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{inactive-Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-G₁=Gx∘Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-G₁=Gx∘Gϱ}\AgdaSpace{}%
\AgdaBound{inactive-Gϱ}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
%
\>[2]\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-one>
\begin{code}%
\>[0]\AgdaComment{-- apply a continuation}\<%
\\
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%<*decompose>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tsp-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</decompose>
%<*decompose-var>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose-one}\AgdaSpace{}%
\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-var>
\begin{code}%
\>[0]\AgdaComment{\{-
decompose tsp ssp-G=G₁∘G₂ (var x) ϱ κ with access ϱ x
... | Gx , Gϱ , inactive-Gϱ , ssp-G₁=Gx∘Gϱ , v 
  rewrite inactive-right-ssplit ssp-G₁=Gx∘Gϱ inactive-Gϱ =
  Ready ssp-G=G₁∘G₂ v κ
-\}}\<%
\\
\>[0]\AgdaComment{-- = apply-cont f ssp κ v}\<%
\end{code}
%<*decompose-unit>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unit}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-unit>
\begin{code}%
\>[0]\AgdaComment{-- = apply-cont f ssp κ (VUnit (inactive-venv unr-Φ ϱ))}\<%
\end{code}
%<*decompose-bind>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ₂}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{split-rotate}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{sp}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁₁,G₁₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-G₁=G₁₁∘G₁₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tsp-Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'-tsp}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{ssp-G₁=G₁₁∘G₁₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁₁∘Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-Gi=G₁₂∘G₂}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp-Φ'}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁₁∘Gi}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{ϱ₁}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{Φ'-tsp}\AgdaSpace{}%
\AgdaBound{ssp-Gi=G₁₂∘G₂}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\<%
\end{code}
%</decompose-bind>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{x₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gv₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-v1r1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gv₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-v2r2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-v1r1}\AgdaSpace{}%
\AgdaBound{ina-Gr₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-v2r2}\AgdaSpace{}%
\AgdaBound{ina-Gr₂}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaComment{--  apply-cont f ssp κ (VPair ss-G1G1'G2' v₁ v₂)}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gvp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-vpr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-GG₁G₂}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-rotate}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{sp}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ts-ΦΦ1Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ts-Φ'Φ3Φ4}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-vpr}\AgdaSpace{}%
\AgdaBound{ina-Gr}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaBound{ss-GG₁G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G3G1Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G2G2'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{ts-Φ'Φ3Φ4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-G3G1Gi}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-G1G2G2'}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%<*decompose-fork>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSymbol{\{}\AgdaArgument{Φ₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{\}\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{split-refl-left}\AgdaSpace{}%
\AgdaBound{Φ₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr-Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ'}\AgdaSpace{}%
\AgdaBound{ϱ₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina-Gp2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaBound{ss-Gp}\AgdaSpace{}%
\AgdaBound{ina-Gp2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ss-Gp'}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaBound{ss-Gp'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-expr}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaBound{ina-Gp2}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-fork>
%<*decompose-new>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{inactive-G₁}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{inactive-G₁}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
%
\>[2]\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-new>
%<*decompose-close>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose-one}\AgdaSpace{}%
\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-close>
{-
decompose tsp ssp-G=G₁∘G₂ (close ch) ϱ κ with access ϱ ch
... | Gx , Gϱ , inactive-Gϱ , ssp-G₁=Gx∘Gϱ , vch
  rewrite inactive-right-ssplit ssp-G₁=Gx∘Gϱ inactive-Gϱ =
  Close ssp-G=G₁∘G₂ vch κ
-}
%<*decompose-wait>
\begin{code}%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose-one}\AgdaSpace{}%
\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\<%
\end{code}
%</decompose-wait>
{-
decompose tsp ssp (wait ch) ϱ κ with access ϱ ch
... | _ , _ , ina , ssp12 , vch rewrite inactive-right-ssplit ssp12 ina = 
  Wait ssp vch κ
-}
\begin{code}%
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaBound{inG}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{inG2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{inG}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{inG2}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GGiG4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GiG1G3}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GGiG4}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-GiG1G3}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaComment{\{-
apply-cont Empty ssp (bind ts ss e₂ ϱ₂ κ) v =
  Ready ssp v (bind ts ss e₂ ϱ₂ κ)
-\}}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{extract-inactive-from-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{extract-inactive-from-cont}\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- lifting through a trivial extension}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaBound{inG}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{inG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{un-t}\<%
\\
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\end{code}
-- threads
%<*ThreadPool>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{tnil}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp-G=G₁∘G₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</ThreadPool>
Tack a task to the end of a thread pool to implement round robin scheduling
%<*tsnoc>
\begin{code}%
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gcmd}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gcmd}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{Gcmd}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{cmd₁}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\end{code}
%</tsnoc>
Append thread pools
\begin{code}%
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaBound{tp1}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- apply the inactive extension to a thread pool}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- find matching wait instruction in thread pool}\<%
\end{code}
%<*vcr-match>
\begin{code}%
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{s₁}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ChannelRef}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{b₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaBound{b₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\end{code}
%</vcr-match>
-- vcr-match () (here-pos ina-G) (here-pos ina-G₁)
%<*vcr-match-impl>
\begin{code}%
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-negpos}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{dual-involution}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\<%
\\
\>[0]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vcr1}\AgdaSpace{}%
\AgdaBound{vcr2}\<%
\\
\>[0]\AgdaCatchallClause{\AgdaFunction{vcr-match}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{ss}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{vcr1}}\AgdaSpace{}%
\AgdaCatchallClause{\AgdaBound{vcr2}}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\end{code}
%</vcr-match-impl>
\begin{code}%
\>[0]\AgdaComment{\{-
vcr-match (ss-left ss) (here-pos \AgdaUnderscore{}) (there \AgdaUnderscore{}) = nothing
vcr-match (ss-left ss) (here-neg \AgdaUnderscore{}) (there \AgdaUnderscore{}) = nothing
vcr-match (ss-right ss) (there \AgdaUnderscore{}) (here-pos \AgdaUnderscore{}) = nothing
vcr-match (ss-right ss) (there \AgdaUnderscore{}) (here-neg \AgdaUnderscore{}) = nothing
-\}}\<%
\end{code}
%<*matchWaitAndGo>
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- close command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{∃}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{)}\<%
\end{code}
%</matchWaitAndGo>
\begin{code}%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaBound{w-vcr}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSymbol{\{}\AgdaArgument{Gc₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{Gc₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{extract-inactive-from-cont}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-int}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaBound{ss-int}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)))}\<%
\end{code}
%<*Outcome>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Outcome}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
%
\>[2]\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\end{code}
%</Outcome>
Thread scheduling
%<*schedule>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Terminated}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{@(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaBound{tp}\<%
\end{code}
%</schedule>
%<*schedule-Fork>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaArgument{G₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1GuG1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G2unit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss-G1GuG1}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G1GuG1}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{))}\<%
\end{code}
%</schedule-Fork>
%<*schedule-Ready>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{))}\<%
\end{code}
%</schedule-Ready>
%<*schedule-Halt>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{inaG}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{inaG}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{tp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{tp'}\<%
\end{code}
%</schedule-Halt>
%<*schedule-New>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}%
\>[2555I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[2555I]%
\>[11]\AgdaSymbol{(}\AgdaFunction{apply-cont}%
\>[2557I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[2557I]%
\>[23]\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
%
\>[23]\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}%
\>[2560I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\<%
\\
\>[.][@{}l@{}]\<[2560I]%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\<%
\\
%
\>[30]\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))))}\<%
\\
%
\>[11]\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{))}\<%
\end{code}
%</schedule-New>
%<*schedule-Close>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tpnext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{Gnext}\AgdaSpace{}%
\AgdaBound{tpnext}\<%
\end{code}
%</schedule-Close>
\begin{code}%
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- start main thread}\<%
\\
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{))}\<%
\end{code}


==> Session3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Session3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Empty}\<%
\\
\>[0]\AgdaComment{-- open import Data.Fin hiding (\AgdaUnderscore{}+\AgdaUnderscore{} ; \AgdaUnderscore{}≤\AgdaUnderscore{})}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{reverse}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Unit}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaOperator{\AgdaRecord{\AgdaUnderscore{}≤\AgdaUnderscore{}}}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{-- open import Data.Vec hiding ( \AgdaUnderscore{}∈\AgdaUnderscore{} ; \AgdaUnderscore{}>>=\AgdaUnderscore{})}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Function}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Syntax3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Channel3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- a value indexed by a *relevant* session context, which is "used up" by the value}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{inaG}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
\>[0]\AgdaComment{\{-
  VInt  : (i : ℕ)
    → (inaG : Inactive G)
    → Val G TInt
-\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-GG₁G₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ce}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vcr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ValidChannelRef}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{ce}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaSymbol{:}%
\>[16]\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaComment{-- inactive-val UInt (VInt i x) = x}\<%
\\
\>[0]\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{unrt₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt₁}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- type environment-indexed value environment}\<%
\\
\>[0]\AgdaComment{-- session context G describes the entire environment, it splits over all (channel) values}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{px}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{px}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- access a value in an indexed environment}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here}\AgdaSpace{}%
\AgdaBound{allUnr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[40]\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{allUnr}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{access}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{inaG₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrX₀}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{inaG₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- non-empty list of value environments for use in a continuation closure}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{CLEnv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{clnil}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{CLEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{clcons}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ*}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ξ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{CLEnv}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ*}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{CLEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ*}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ssp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ssp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- split environment according to type context split}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{\}}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSymbol{\{}\AgdaArgument{G}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}%
\>[34]\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{unrt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi-1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GGiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[2]\AgdaKeyword{let}\AgdaSpace{}%
\AgdaBound{p₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaBound{unr-v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{in}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[17]\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{rewrite-ssplit}\AgdaSpace{}%
\AgdaBound{p₂}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSymbol{\{}\AgdaArgument{G}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G1'}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose4}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp12}\<%
\\
\>[0]\AgdaSymbol{...|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1'Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-GG1'Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp-GiG1G2'}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\\
%
\>[2]\AgdaInductiveConstructor{More}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Gas}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{mutual}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{(}\AgdaBound{un-Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{un-t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\>[2]\AgdaComment{\{-
    cont : 
      (ϱ : VEnv G Φ)
      → (c : ∀ \{G' Gx\} → SSplit G' Gx G → Val Gx t → VEnv G Φ →  Command G')
      → Cont G Φ t
  -\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ts}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%<*Command-Ready>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Ready>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaSymbol{:}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[4]\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[4]\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[4]\AgdaInductiveConstructor{Wait}%
\>[10]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%<*Command-Send>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{v}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Send>
%<*Command-Recv>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Recv>
%<*Command-Select>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Select>
%<*Command-Branch>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[4][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{dcont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\end{code}
%</Command-Branch>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaComment{-- }\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{rewrite-helper}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G''}\AgdaSpace{}%
\AgdaBound{Φ'}\<%
\\
\>[0]\AgdaFunction{rewrite-helper}\AgdaSpace{}%
\AgdaBound{ina-G2}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ssp-GGG''}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\AgdaSpace{}%
\AgdaBound{ina-G2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{rewrite-ssplit1}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{sym}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ssp-GG1G2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp-GGG''}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{Φ₁}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gx}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaComment{-- decompose tsp ssp (nat unr-Φ i) ϱ κ =}\<%
\\
\>[0]\AgdaComment{--   Ready ssp (VInt i (inactive-venv unr-Φ ϱ)) κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{split-rotate}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{sp}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-G1G2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tsp-Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'-tsp}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ssp-G1G2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-3i}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp-42}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp-Φ'}\AgdaSpace{}%
\AgdaBound{ssp-3i}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSpace{}%
\AgdaBound{ϱ₁}\<%
\\
%
\>[2]\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{Φ'-tsp}\AgdaSpace{}%
\AgdaBound{ssp-42}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{x₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gv₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-v1r1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gv₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-v2r2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-v1r1}\AgdaSpace{}%
\AgdaBound{ina-Gr₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-v2r2}\AgdaSpace{}%
\AgdaBound{ina-Gr₂}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{p}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gvp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-vpr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-GG₁G₂}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-rotate}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{sp}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ts-ΦΦ1Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ts-Φ'Φ3Φ4}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-vpr}\AgdaSpace{}%
\AgdaBound{ina-Gr}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaBound{ss-GG₁G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G3G1Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G2G2'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{ts-Φ'Φ3Φ4}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-G3G1Gi}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-G1G2G2'}\AgdaSpace{}%
\AgdaBound{v₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSymbol{\}\{}\AgdaBound{Φ₁}\AgdaSymbol{\}\{}\AgdaArgument{G}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{\}\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{split-refl-left}\AgdaSpace{}%
\AgdaBound{Φ₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr-Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gp1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gp2}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gp}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ'}\AgdaSpace{}%
\AgdaBound{ϱ₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina-Gp2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit-transform}\AgdaSpace{}%
\AgdaBound{ss-Gp}\AgdaSpace{}%
\AgdaBound{ina-Gp2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ss-Gp'}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-function2}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaBound{ss-Gp'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{sp-ΦΦΦ'}\AgdaSpace{}%
\AgdaBound{ss-g1g1g2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-expr}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaBound{unr-Φ'}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{unr-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gch}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{vch'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{vch'}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gch}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gϱ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ssp12}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{vch'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{vch'}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{vv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gg}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₄}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G₄}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g3g4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{vv}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₅}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₆}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G₆}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2g5g6}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vvv}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-gg}\AgdaSpace{}%
\AgdaBound{ss-g1g3g4}\AgdaSpace{}%
\AgdaBound{ss-g2g5g6}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1'g2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3g5}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g6}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-g1g3g4}\AgdaSpace{}%
\AgdaBound{ina-G₄}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{sym}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-g2g5g6}\AgdaSpace{}%
\AgdaBound{ina-G₆}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ss-gg}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{vvv}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{select}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{branch}\AgdaSymbol{\{}\AgdaBound{s₁}\AgdaSymbol{\}\{}\AgdaBound{s₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{e-left}\AgdaSpace{}%
\AgdaBound{e-rght}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-env}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ϱ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{access}\AgdaSpace{}%
\AgdaBound{ϱ₁}\AgdaSpace{}%
\AgdaBound{ch}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ss-G1G1'G2'}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G-G1'Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi-G2'-G2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split-rotate}\AgdaSpace{}%
\AgdaBound{tsp}\AgdaSpace{}%
\AgdaBound{sp}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp-ΦΦ1Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp-Φ'Φ3Φ4}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-right-ssplit}\AgdaSpace{}%
\AgdaBound{ss-vi}\AgdaSpace{}%
\AgdaBound{ina-G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss-G-G1'Gi}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaFunction{dcont}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaFunction{dcont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{))}\<%
\\
%
\>[4]\AgdaFunction{dcont}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{sp-Φ'Φ3Φ4}\AgdaSpace{}%
\AgdaBound{ss-Gi-G2'-G2}\AgdaSpace{}%
\AgdaBound{e-left}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
%
\>[4]\AgdaFunction{dcont}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{sp-Φ'Φ3Φ4}\AgdaSpace{}%
\AgdaBound{ss-Gi-G2'-G2}\AgdaSpace{}%
\AgdaBound{e-rght}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- apply a continuation}\<%
\\
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaBound{un-Φ}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{inactive-venv}\AgdaSpace{}%
\AgdaBound{un-Φ}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-val}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{v}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{inG1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{inG2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{inG2}\AgdaSpace{}%
\AgdaBound{inG1}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GGiG4}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GiG1G3}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GGiG4}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ss-GiG1G3}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{extract-inactive-from-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{extract-inactive-from-cont}\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- lifting through a trivial extension}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{-- lift-val (VInt i x) = VInt i (ina-:: \AgdaUnderscore{} x)}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{VEnv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{vcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ssp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaBound{un-Φ}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaBound{un-Φ}\AgdaSpace{}%
\AgdaBound{un-t}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaBound{ϱ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{bind}\AgdaSpace{}%
\AgdaBound{ts}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-venv}\AgdaSpace{}%
\AgdaBound{ϱ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-val}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{dcont}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{-- threads}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Inactive}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- tack a task to the end of a thread pool to implement round robin scheduling}\<%
\\
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gpool}\AgdaSpace{}%
\AgdaBound{Gcmd}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gcmd}\AgdaSpace{}%
\AgdaBound{Gpool}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gpool}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Command}\AgdaSpace{}%
\AgdaBound{Gcmd}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{cmd₁}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- append thread pools}\<%
\\
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G1}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G2}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{tp2}\<%
\\
\>[0]\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-rec}\AgdaSpace{}%
\AgdaBound{tp1}\AgdaSpace{}%
\AgdaBound{tp2}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- reverse thread pool}\<%
\\
\>[0]\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[0]\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\<%
\\
\>[0]\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{treverse}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cmd}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- apply the inactive extension to a thread pool}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ina-::}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-both}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-command}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- close command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}%
\>[37]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{cl-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaBound{w-vcr}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchWaitAndGo}\AgdaSymbol{\{}\AgdaArgument{Gc₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-cl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{cl-b}\AgdaSpace{}%
\AgdaBound{cl-vcr}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{w-b}\AgdaSpace{}%
\AgdaBound{w-vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g3gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gchannels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-top'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-channels}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right-inactive}\AgdaSpace{}%
\AgdaBound{Gc₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{extract-inactive-from-cont}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaBound{κ}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-Gunit'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-stopped'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gtpacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-g4g2}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-int}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose2}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-others}\AgdaSpace{}%
\AgdaBound{ss-int}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gother}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-sym}\AgdaSpace{}%
\AgdaBound{ss-other}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-outer-cons}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{cl-κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-g2gacc}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-stopped'}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaBound{ina-Gunit'}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- read command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-arg}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}%
\>[86]\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}%
\>[75]\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSymbol{@(}\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi'gig2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi''gi'gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi''}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gg1'g2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1'gc1g11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2'gc2gi''}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-gg1'g2'}\AgdaSpace{}%
\AgdaBound{ss-g1'gc1g11}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaBound{vcr}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaComment{\{-t1≡t-\}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds1≡s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-out1}\AgdaSpace{}%
\AgdaBound{ss-out2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gi''gi'gtpacc}\AgdaSpace{}%
\AgdaBound{ss-gi'gig2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GSi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi''GiGi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi1G2Gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-out1}\AgdaSpace{}%
\AgdaBound{ss-out2}\AgdaSpace{}%
\AgdaBound{ss-g2'gc2gi''}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GG1'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1'-GG2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG1'-GG11-Gc2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2'-G12-Gi''}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-rotate}\AgdaSpace{}%
\AgdaBound{ss-GG2'-G12-Gi''}\AgdaSpace{}%
\AgdaBound{ss-Gi''GiGi1}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi''+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gi+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2-G12-Gi''+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi''+Gi+Gsi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gi+-G12-G4}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1'-GG2'}\AgdaSpace{}%
\AgdaBound{ss-GG1'-GG11-Gc2}\AgdaSpace{}%
\AgdaBound{ss-GG2-G12-Gi''+}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GG1''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG2''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1''-GG2''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG1''-GG11-G12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG2''-Gc2-Gi''+}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-GG-GG1''-GG2''}\AgdaSpace{}%
\AgdaBound{ss-GG2''-Gc2-Gi''+}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-Gii-Gi''+}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-Gii-GG1''-Gc2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}%
\>[59]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-GG-Gii-Gi''+}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-Gii-GG1''-Gc2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaBound{ss-GG1''-GG11-G12}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr-recv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-Gi''+Gi+Gsi}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-Gi+-G12-G4}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr-send}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-Gi1G2Gtpacc}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{))))}\<%
\\
\>[0]\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSymbol{@(}\AgdaBound{ss-rv}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ-rv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1g11gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gig12g3}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwlg11g2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi'gig2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpg11gi''}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi''gi'gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G₁'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{G₂'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gg1'g2'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g1'gc1g11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g2'gc2gi''}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi0}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{recv-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gtp}\<%
\\
%
\>[2]\AgdaComment{-- select command}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gc}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Val}\AgdaSpace{}%
\AgdaBound{Gc₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Cont}\AgdaSpace{}%
\AgdaBound{Gc₂}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)))}\<%
\\
%
\>[2]\AgdaComment{-- focused thread pool}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{SSplit}\AgdaSpace{}%
\AgdaBound{Gtp}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaBound{Gtpacc}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpwl}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{Gtpacc}\<%
\\
%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Maybe}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Fork}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{ss-args}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose6}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc'-gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc'-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp'-gc2-gi1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{vcr-match-2-sb}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss-g-gc'-gtp'}\AgdaSpace{}%
\AgdaBound{ss-gc'-gc1-g1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSpace{}%
\AgdaBound{lab}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSymbol{@(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc'-gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc'-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp'-gc2-gi1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose5}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaBound{ss}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gix}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaBound{select-info}\AgdaSpace{}%
\AgdaBound{ss-tp'}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss'}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss-top}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtpwl-g3-gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp-g3-gi1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gc'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-g-gc'-gtp'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gc'-gc1-g1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gtp'-gc2-gi1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ds3=s1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ds4=s2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG11}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GG12}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{junction}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSpace{}%
\AgdaBound{ss2'}%
\>[332]\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-sel}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vcr-bra}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss-gi1-gi-gtpacc}\AgdaSpace{}%
\AgdaBound{ss-gi-g4-g2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi1-g3-gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi2-g2-gtpacc}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-join}\AgdaSpace{}%
\AgdaBound{ss1'}\AgdaSpace{}%
\AgdaBound{ss2'}\AgdaSpace{}%
\AgdaBound{ss-gtp'-gc2-gi1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{GGG1}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{GGG2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG-ggg1-ggg2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg1-gc1-gc2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-g1-gi1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose3}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-g1-gi1}\AgdaSpace{}%
\AgdaBound{ss-gi1-g3-gi2}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi3}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-ggg2-gi3-gi2}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-gi3-gg12-g2}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{GG}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-GG-ggg1-ggg2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-ggg1-gc1-gc2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b₁}\AgdaSpace{}%
\AgdaBound{vcr-sel}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss-ggg2-gi3-gi2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss-gi3-gg12-g2}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaBound{b}\AgdaSpace{}%
\AgdaBound{vcr-bra}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{dcont}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tappend}\AgdaSpace{}%
\AgdaBound{ss-gi2-g2-gtpacc}\AgdaSpace{}%
\AgdaBound{tp-wl}\AgdaSpace{}%
\AgdaBound{tp-acc}\AgdaSymbol{)))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Outcome}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Terminated}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
%
\>[2]\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- thread scheduling}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{ThreadPool}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{Terminated}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Fork}\AgdaSymbol{\{}\AgdaArgument{G₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaArgument{G₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-compose}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{ss₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gunit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G2unit}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₁₃}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSpace{}%
\AgdaBound{κ₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G1GunitG1}\AgdaSymbol{)))}\<%
\\
%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss₂₄}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSpace{}%
\AgdaBound{κ₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-G2GuG2}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Ready}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaBound{ss₁}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{inaG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{inactive-left-ssplit}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{inaG}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Halt}\AgdaSpace{}%
\AgdaBound{inaG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{tp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{tp'}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{New}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-right}\AgdaSpace{}%
\AgdaBound{G₁}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Gi}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-inactive-right}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}%
\>[4290I]\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[4290I]%
\>[11]\AgdaSymbol{(}\AgdaFunction{apply-cont}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-left}\AgdaSpace{}%
\AgdaBound{ss-GiG1}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift-cont}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{ss-posneg}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{inactive-ssplit-trivial}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-pos}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{VChan}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{here-neg}\AgdaSpace{}%
\AgdaBound{ina-Gi}\AgdaSymbol{))))}\<%
\\
%
\>[11]\AgdaSymbol{(}\AgdaFunction{lift-threadpool}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{))}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchWaitAndGo}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Gnext}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tpnext}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{Gnext}\AgdaSpace{}%
\AgdaBound{tpnext}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Close}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Wait}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Send}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchSendAndGo}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G-next}\AgdaSpace{}%
\AgdaBound{tp-next}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Recv}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{v}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{ssplit-refl-left-inactive}\AgdaSpace{}%
\AgdaBound{G₂}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{matchBranchAndGo}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{G-next}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{tp-next}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G-next}\AgdaSpace{}%
\AgdaBound{tp-next}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₁}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Select}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{κ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ina-G'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{ss-GG'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{More}\AgdaSpace{}%
\AgdaBound{f}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{@(}\AgdaInductiveConstructor{Branch}\AgdaSpace{}%
\AgdaBound{ss-vκ}\AgdaSpace{}%
\AgdaBound{vch}\AgdaSpace{}%
\AgdaBound{dcont}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{tsnoc}\AgdaSpace{}%
\AgdaBound{ss}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSpace{}%
\AgdaBound{cmd}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaInductiveConstructor{Empty}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{tp}\AgdaSymbol{@(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{})}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{OutOfGas}\AgdaSpace{}%
\AgdaBound{tp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- start main thread}\<%
\\
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Gas}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Outcome}\<%
\\
\>[0]\AgdaFunction{start}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{=}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaFunction{schedule}\AgdaSpace{}%
\AgdaBound{f}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tcons}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{decompose}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{ss-[]}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{halt-cont}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{vnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{)))}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{tnil}\AgdaSpace{}%
\AgdaInductiveConstructor{ina-[]}\AgdaSymbol{))}\<%
\end{code}


==> Syntax0.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Syntax0}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{reverse}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing0}\<%
\end{code}
Expressions
%<*expr-all>
%<*expr-var>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</expr-var>
%<*expr-unit>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{unit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\end{code}
%</expr-unit>
%<*expr-pair>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\end{code}
%</expr-pair>
%<*expr-bind>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\end{code}
%</expr-bind>
%<*expr-fork>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{a}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)))}\<%
\\
%
\>[2]\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\end{code}
%</expr-fork>
%</expr-all>
\begin{code}%
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{tᵤ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{tᵤ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tᵤ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unit}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{unit}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e₁}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{e}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\end{code}


==> Syntax3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Syntax3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{reverse}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{selection}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{A}\<%
\\
\>[0]\AgdaFunction{selection}\AgdaSpace{}%
\AgdaInductiveConstructor{Left}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{selection}\AgdaSpace{}%
\AgdaInductiveConstructor{Right}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{y}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaOperator{\AgdaFunction{\AgdaUnderscore{}≜\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\<%
\\
\>[0]\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} expressions}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{var}%
\>[68I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[.]\<[68I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaComment{\{{-}
  nat : (unr{-}Φ : All Unr Φ)
      → (i : ℕ)
      → Expr Φ TInt
{-}\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{new}%
\>[174I]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unr{-}Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
\>[.]\<[174I]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)))}\<%
\end{code}
%<*Expr-send>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\end{code}
%</Expr-send>
%<*Expr-recv>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{))}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\end{code}
%</Expr-recv>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{select}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Selector}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{selection}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{))}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\>[2]\AgdaInductiveConstructor{branch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{sp}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{eleft}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{erght}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
%
\>[6]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\<%
\end{code}
\begin{code}%
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{tᵤ}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{tᵤ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Expr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{tᵤ}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{var}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaComment{{-}{-}lift{-}expr unrtu (nat unr{-}Φ i) = nat (unrtu ∷ unr{-}Φ) i}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{e}\AgdaSpace{}%
\AgdaBound{e₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{letbind}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e₁}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{pair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{letpair}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{e}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{fork}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{e}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{new}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{close}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{wait}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{vv}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{send}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{vv}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{recv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{select}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{select}\AgdaSpace{}%
\AgdaBound{lab}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{lift{-}expr}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{branch}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{branch}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaBound{unrtu}\AgdaSpace{}%
\AgdaBound{ch}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{x₂}\<%
\end{code}


==> TypeReduction3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{TypeReduction3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\AgdaSpace{}%
\AgdaKeyword{hiding}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{map}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Maybe}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Typing3}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Global3}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{-- Reduction of the session context}\<%
\end{code}
%<*type-reduction-internal>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}⇒′\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{RedThere}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaBound{e}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{e}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{RedEnd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{nothing}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{RedTransmit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{\}}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}%
\>[60I]\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[.][@{}l@{}]\<[60I]%
\>[12]\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\end{code}
%</type-reduction-internal>
\begin{code}%
%
\>[2]\AgdaInductiveConstructor{RedChLeft}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s₁}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{RedChRight}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s₂}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
\>[0]\<%
\end{code}
%<*type-reduction>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}⇒\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{SCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{RedIdent}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒}}\AgdaSpace{}%
\AgdaBound{G}\<%
\\
%
\>[2]\AgdaInductiveConstructor{RedNew}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{just}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{POSNEG}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{G}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{RedInternal}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{G′}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒′}}\AgdaSpace{}%
\AgdaBound{G′}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{G}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⇒}}\AgdaSpace{}%
\AgdaBound{G′}\<%
\end{code}
%</type-reduction>


==> Typing0.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Typing0}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} specific}\<%
\end{code}
%<*Polarity>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Polarity}\<%
\\
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\<%
\\
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\<%
\end{code}
%</Polarity>
Types and session types
%<*types>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\<%
\\
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\>[2]\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\>[2]\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\end{code}
%</types>
%<*dual>
\begin{code}%
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\<%
\\
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{dual{-}involution}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{dual{-}involution}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{dual{-}involution}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}
%</dual>
\begin{code}%
\>[0]\<%
\\
\>[0]\AgdaFunction{xdual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Bool}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
\>[0]\AgdaFunction{xdual}\AgdaSpace{}%
\AgdaInductiveConstructor{false}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{xdual}\AgdaSpace{}%
\AgdaInductiveConstructor{true}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} linear and unrestricted types}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{LChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\end{code}
%<*unr>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\end{code}
%</unr>
\begin{code}%
\>[0]\AgdaComment{{-}{-} lin and unr are mutually exclusive}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSpace{}%
\AgdaBound{x₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}%
\>[19]\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{lin}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{lin}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{lin}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSpace{}%
\AgdaBound{lin}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} should be expressible by pattern matching lambda, but ...}\<%
\\
\>[0]\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{u₁}\AgdaSpace{}%
\AgdaBound{u₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{u₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{u₁}\AgdaSpace{}%
\AgdaBound{u₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{u₂}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Dec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{ltp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{ltp}\<%
\\
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{ltp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaBound{ltp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Dec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{y₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\<%
\end{code}
Context splitting, respecting linearity
%<*splitting>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≜\AgdaUnderscore{}∘\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\>[2]\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≜}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∘}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\end{code}
%</splitting>
\begin{code}%
\>[0]\AgdaFunction{Split}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}≜\AgdaUnderscore{}∘\AgdaUnderscore{}}}\<%
\\
\>[0]\AgdaComment{{-}{-} split the unrestricted part from a typing context}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ'}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp'}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{sp'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} reorganize splits}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaFunction{Split}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{lft}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rgt}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\end{code}
Extract from type context where all other entries are unrestricted
%<*element>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}∈\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{t₀}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₀}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t₀}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\<%
\end{code}
%</element>


==> Typing3.tex <==
\begin{code}%
\>[0]\AgdaKeyword{module}\AgdaSpace{}%
\AgdaModule{Typing3}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Bool}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.List.All}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Fin}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Nat}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Product}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Data.Sum}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Nullary}\<%
\\
\>[0]\AgdaKeyword{open}\AgdaSpace{}%
\AgdaKeyword{import}\AgdaSpace{}%
\AgdaModule{Relation.Binary.PropositionalEquality}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Polarity}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Polarity}\<%
\\
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\<%
\\
\>[0]\AgdaFunction{otherEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{NEG}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{POS}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} types and session types}\<%
\end{code}
%<*types>
\begin{code}%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{mutual}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\>[4]\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\>[4]\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
%
\>[2]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[2][@{}l@{\AgdaIndent{0}}]%
\>[4]\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
%
\>[4]\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\end{code}
%</types>
\begin{code}%
%
\>[4]\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s₁}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{s₂}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SIntern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SExtern}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\<%
\\
\>[0]\<%
\end{code}
%<*sty-patterns>
\begin{code}%
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SSend}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\<%
\\
\>[0]\AgdaKeyword{pattern}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd?}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\<%
\end{code}
%</sty-patterns>
%<*async>
\begin{code}%
\>[0]\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\\
\>[0]\AgdaFunction{AChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SRecv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd!}\AgdaSymbol{)}\<%
\end{code}
%</async>
%<*dual-dir>
\begin{code}%
\>[0]\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Dir}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Dir}\<%
\\
\>[0]\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\<%
\\
\>[0]\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\<%
\end{code}
%</dual-dir>
%<*dual-dir-inv>
\begin{code}%
\>[0]\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{d}\<%
\\
\>[0]\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaInductiveConstructor{SND}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaInductiveConstructor{RCV}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}
%</dual-dir-inv>
%<*dual>
\begin{code}%
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{STy}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{STy}\<%
\\
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\<%
\end{code}
%</dual>
\begin{code}%
\>[0]\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual{-}dir}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\<%
\end{code}
%<*dual-inv>
\begin{code}%
\>[0]\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{dual}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{dual}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{≡}}\AgdaSpace{}%
\AgdaBound{s}\<%
\\
\>[0]\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{STrm}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaBound{s}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
\>[0]\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SEnd}\AgdaSpace{}%
\AgdaBound{d}\AgdaSymbol{)}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\end{code}
%</dual-inv>
\begin{code}%
\>[0]\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{SCho}\AgdaSpace{}%
\AgdaBound{d}%
\>[18]\AgdaBound{s₁}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{rewrite}\AgdaSpace{}%
\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaBound{s₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{dual{-}inv}\AgdaSpace{}%
\AgdaBound{s₂}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{dual{-}dir{-}inv}\AgdaSpace{}%
\AgdaBound{d}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{refl}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} linear and unrestricted types}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{LChan}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{s}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{s}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\<%
\\
%
\>[2]\AgdaComment{{-}{-} UInt : Unr TInt}\<%
\\
%
\>[2]\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} lin and unr are mutually exclusive}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSpace{}%
\AgdaBound{x}\<%
\\
\>[0]\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}lin{-}unr}\AgdaSpace{}%
\AgdaBound{lint}\AgdaSpace{}%
\AgdaBound{x₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}%
\>[19]\AgdaSymbol{\{}\AgdaBound{t}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\AgdaSpace{}%
\AgdaSymbol{()}\<%
\\
\>[0]\AgdaComment{{-}{-} lemma{-}unr{-}lin UInt ()}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{lin}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{lin}\<%
\\
\>[0]\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{unr}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{lin}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaFunction{lemma{-}unr{-}lin}\AgdaSpace{}%
\AgdaBound{unr₁}\AgdaSpace{}%
\AgdaBound{lin}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} should be expressible by pattern matching lambda, but ...}\<%
\\
\>[0]\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{u₁}\AgdaSpace{}%
\AgdaBound{u₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{u₁}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{u₁}\AgdaSpace{}%
\AgdaBound{u₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{u₂}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Dec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\<%
\\
\>[0]\AgdaComment{{-}{-} unrestricted{-}type TInt = yes UInt}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}right}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}left}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{unrestricted{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{¬}}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{ltp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{ltp}\<%
\\
\>[0]\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬l₁}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{ltp}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{¬l₂}\AgdaSpace{}%
\AgdaBound{ltp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Dec}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(λ}\AgdaSpace{}%
\AgdaSymbol{())}\<%
\\
\>[0]\AgdaComment{{-}{-} linear{-}type TInt = no (λ ())}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaBound{p}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{p}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{no}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaFunction{destroy{-}both}\AgdaSpace{}%
\AgdaBound{¬p}\AgdaSpace{}%
\AgdaBound{¬p₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{linear{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{yes}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Lin}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{⊎}}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaInductiveConstructor{TUnit}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaInductiveConstructor{UUnit}\<%
\\
\>[0]\AgdaComment{{-}{-} classify{-}type TInt = inj₂ UInt}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t₂}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair1}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{LPair2}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TPair}\AgdaSpace{}%
\AgdaBound{t₁}\AgdaSpace{}%
\AgdaBound{t₂}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y₁}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{UPair}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{y₁}\AgdaSymbol{)}\<%
\\
\>[0]\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{TChan}\AgdaSpace{}%
\AgdaBound{x}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaInductiveConstructor{LChan}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} typing context}\<%
\end{code}
%<*TCtx>
\begin{code}%
\>[0]\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\<%
\\
\>[0]\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaDatatype{List}\AgdaSpace{}%
\AgdaDatatype{Ty}\<%
\end{code}
%</TCtx>
\begin{code}%
\>[0]\AgdaComment{{-}{-} context splitting, respecting linearity}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
%
\>[2]\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
%
\>[2]\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{t}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSymbol{)}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} split the unrestricted part from a typing context}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ'}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaFunction{classify{-}type}\AgdaSpace{}%
\AgdaBound{t}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₁}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp'}\<%
\\
\>[0]\AgdaFunction{split{-}refl{-}left}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp'}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaInductiveConstructor{inj₂}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{t}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{unr{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{y}\AgdaSpace{}%
\AgdaBound{sp'}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} reorganize splits}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSymbol{\}}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ₁}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaRecord{Σ}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{λ}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ}\AgdaSpace{}%
\AgdaBound{Φ₁₁}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaFunction{×}}\AgdaSpace{}%
\AgdaDatatype{Split}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaBound{Φ₁₂}\AgdaSpace{}%
\AgdaBound{Φ₂}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{[]}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{unr}\AgdaSpace{}%
\AgdaBound{x₁}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{left}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
\>[0]\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaBound{sp1112}\AgdaSpace{}%
\AgdaKeyword{with}\AgdaSpace{}%
\AgdaFunction{split{-}rotate}\AgdaSpace{}%
\AgdaBound{sp12}\AgdaSpace{}%
\AgdaBound{sp1112}\<%
\\
\>[0]\AgdaSymbol{...}\AgdaSpace{}%
\AgdaSymbol{|}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\AgdaSpace{}%
\AgdaSymbol{=}\AgdaSpace{}%
\AgdaSymbol{\AgdaUnderscore{}}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{sp{-}Φ'}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{,}}\AgdaSpace{}%
\AgdaInductiveConstructor{rght}\AgdaSpace{}%
\AgdaBound{Φ'{-}sp}\<%
\\
%
\\[\AgdaEmptyExtraSkip]%
\>[0]\AgdaComment{{-}{-} extract from type context where all other entries are unrestricted}\<%
\\
\>[0]\AgdaKeyword{data}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{\AgdaUnderscore{}∈\AgdaUnderscore{}}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaDatatype{Ty}\AgdaSymbol{)}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaFunction{TCtx}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaPrimitiveType{Set}\AgdaSpace{}%
\AgdaKeyword{where}\<%
\\
\>[0][@{}l@{\AgdaIndent{0}}]%
\>[2]\AgdaInductiveConstructor{here}%
\>[8]\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{All}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSymbol{)}\<%
\\
%
\>[2]\AgdaInductiveConstructor{there}\AgdaSpace{}%
\AgdaSymbol{:}\AgdaSpace{}%
\AgdaSymbol{∀}\AgdaSpace{}%
\AgdaSymbol{\{}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSpace{}%
\AgdaSymbol{\}}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaDatatype{Unr}\AgdaSpace{}%
\AgdaBound{x₀}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSpace{}%
\AgdaSymbol{→}\AgdaSpace{}%
\AgdaBound{x}\AgdaSpace{}%
\AgdaOperator{\AgdaDatatype{∈}}\AgdaSpace{}%
\AgdaSymbol{(}\AgdaBound{x₀}\AgdaSpace{}%
\AgdaOperator{\AgdaInductiveConstructor{∷}}\AgdaSpace{}%
\AgdaBound{xs}\AgdaSymbol{)}\<%
\end{code}

